Geometric Insights into Focal Loss: Reducing Curvature for Enhanced Model Calibration

The key factor in implementing machine learning algorithms in decision-making situations is not only the accuracy of the model but also its confidence level. The confidence level of a model in a classification problem is often given by the output vector of a softmax function for convenience. However, these values are known to deviate significantly from the actual expected model confidence. This problem is called model calibration and has been studied extensively. One of the simplest techniques to tackle this task is focal loss, a generalization of cross-entropy by introducing one positive parameter. Although many related studies exist because of the simplicity of the idea and its formalization, the theoretical analysis of its behavior is still insufficient. In this study, our objective is to understand the behavior of focal loss by reinterpreting this function geometrically. Our analysis suggests that focal loss reduces the curvature of the loss surface in training the model. This indicates that curvature may be one of the essential factors in achieving model calibration. We design numerical experiments to support this conjecture to reveal the behavior of focal loss and the relationship between calibration performance and curvature.

==> section/conjectures.tex <==
% \vspace{1mm}
% \vspace{-2mm}
\section{Empirical remarks and conjectures}
% \vspace{-2mm}
\label{sec:conjectures}
% \vspace{-1mm}

Our experimental framework incorporated two types of tasks: sampling bias tasks and domain generalization tasks. For the sampling bias tasks, models were trained on CIFAR10 \citep{Krizhevsky09learningmultiple} and tested on CIFAR10.1 \citep{recht2018cifar10.1}, and analogously, we trained on ImageNet-1K \citep{russakovsky2015imagenet} and tested on ImageNet-V2 \citep{recht2019imagenet}. For the domain generalization tasks, we employed the DomainBed datasets \citep{Gulrajani21}, with our experiments specifically addressing PACS \citep{li2017deeper} and VLCS \citep{fang2013unbiased} tasks. Detailed information about our experimental setup is available in Appendix \ref{appendix:exp_setting}.

In terms of the performance of SAM and Focal Loss, we found SAM, controlled by the regularization intensity parameter $\rho$, and Focal Loss, controlled by $\gamma$, to exhibit distinct behaviors.
Based on our previous discussions and experimental results, we can provide the following empirical remarks and conjectures.

\begin{remark}[informal]
% Fig1
    SAM effectively resolves the tradeoff between OOD generalization and calibration performance w.r.t. curvature (see Figure~\ref{fig:fig1}). %SAM demonstrated improvements in curvature and effectively resolved this tradeoff (see Figure \ref{fig:fig1}). 
\end{remark}

\begin{remark}[informal]
% Fig2
    From Figure~\ref{fig:fig2}, we have,
    %\begin{itemize}
        %\item[i)]
        i) SAM controls OOD generalization and ECE with curvature via parameter $\rho$;
        %\item[ii)]
        ii) Focal loss cannot improve curvature relatively and fails to resolve the tradeoff with parameter $\gamma$.
    %\end{itemize}
    %$\rho$ was shown to control curvature, which in turn influenced OOD generalization and ECE. In contrast, Focal Loss was unable to improve curvature or resolve the tradeoff, improving one aspect only at the expense of the other. $\gamma$ only served to control ECE (see Figure \ref{fig:fig2}).
\end{remark}


\begin{conjecture}
% Fig3
    In a practical case,
    %\begin{itemize}
        %\item[i)]
        i) 1-batch SAM generates large variance curvature.
    full-batch SAM reduces curvature;
        %\item[ii)]
        ii) Full-batch SAM reduces curvature, improves ECE, and cannot improve ACC relatively.
    %\end{itemize}
    Then, the existence of an optimal BS can be expected (see Figure~\ref{fig:fig3}, BS=256 is optimal compared to BS=1 and BS=full).
    % Moreover, we noted variations in behavior based on Batch Size (BS), with the most extreme cases not necessarily resulting in the greatest curvature improvements.
    % Whatever batch size is used, training with SAM reduces SR(H) and Laplacian(H). However,  the only setting of BS=1 failed to suppress ECE.

    
\end{conjecture}


\begin{conjecture}
    If the loss landscape is locally convex, 1-batch SAM and focal loss behave similarly.
\end{conjecture}

==> section/curvature_and_contractions.tex <==

% \vspace{-2mm}
\section{Curvature and contractions}
% \vspace{-2mm}
\label{sec:curvature_and_contractions}
In many literatures, the Hessian is often regarded as the curvature of the manifold or the loss landscape and is utilized in discussions of various behaviors of neural networks~\citep{martens2015optimizing,gilmer2021loss,osawa2019large,martens2018kronecker}.
Specifically, the trace and eigenvalues of the Hessian are commonly used as approximations.
To begin with, we first organize the role of these approximations in relation to curvature.

Throughout the manuscript, the Einstein summation convention is assumed, so that summation will be automatically taken over indices repeated twice in the term, e.g., $\bm{a}^i\bm{b}_i = \sum_{i} a^ib_i$.
See Appendix~\cref{apd:geometry} and textbooks on Riemannian manifolds and differential geometry~\citep{lee2018introduction,kuhnel2015differential,guggenheimer2012differential,lee2006riemannian} for details on the terminology related to differential geometry.

Let $(\mathcal{M}, \mathfrak{g})$ be the Riemannian manifold with metric $\mathfrak{g}$.
For example, if we consider the manifold of neural networks, $\mathcal{M}$ is the set of neural networks parametrized $\bm{\theta} \in \mathbb{R}^d$ for $d \in [0, \infty)$.
\begin{definition}
    \label{def:vector_field}
    A vector field $X$ on manifold $\mathcal{M}$ is a smooth map $X$ that assigns to each point $p \in \mathcal{M}$ a vector $X_p$ in $T_p\mathcal{M}$, where $T_p\mathcal{M}$ is the tangent space of $\mathcal{M}$ at $p$.
    For any function $f \in \mathcal{F}(\mathcal{M})$ we define the real-valued function $(Xf)_p = X_p f$, and it is called smooth if $Xf \in \mathcal{F}(\mathcal{M})$.
    The set of all vector fields on $\mathcal{M}$ will be denoted by $\mathcal{X}(\mathcal{M})$.
\end{definition}
\begin{definition}
\label{def:curvature}
    The curvature of the linear connection $\nabla$ is
    \small
    \begin{align}
        R: \mathcal{X}(\mathcal{M})\times\mathcal{X}(\mathcal{M})\times\mathcal{X}(\mathcal{M}) \to \mathcal{X}(\mathcal{M}), \nonumber \\
        R(X, Y, Z) \coloneqq \nabla_X\nabla_YZ - \nabla_Y\nabla_XZ - \nabla_{[X, Y]}Z,
    \end{align}
    \normalsize
    for $X, Y, Z \in \mathcal{X}(\mathcal{M})$ and $[X, Y]$ is the Lie Bracket.
\end{definition}
On a Riemannian manifold, it is known that there exists a unique torsion-free, metric connection $\nabla$ called Levi-Civita connection, and its associated connection coefficients are
% \vspace{-2mm}
\small
\begin{align}
    \Gamma^l_{ij} \coloneqq \frac{1}{2}\mathfrak{g}^{lk}(\frac{\partial}{\partial\theta_i}\mathfrak{g}_{jk} + \frac{\partial}{\partial\theta_j}\mathfrak{g}_{ik} - \frac{\partial}{\partial\theta_k}\mathfrak{g}_{ij}),
\end{align}
\normalsize
where $(\mathfrak{g}^{lk})$ denotes the inverse matrix of $(\mathfrak{g}_{ij})$.
The coordinates $\Gamma^l_{ij}$ of the Levi-Civita connection are called the Christoffel symbols.
Here, the curvature tensor associated with the Levi-Civita connection is called the Riemannian curvature tensor, and it can be expressed as
\small
\begin{align}
    R^r_{ijk} \coloneqq \frac{\partial}{\partial_i}\Gamma^r_{jk} - \frac{\partial}{\partial_j}\Gamma^r_{ik} + \Gamma^r_{il}\Gamma^l_{jk} - \Gamma^r_{jl}\Gamma^l_{ik}. \label{eq:riemannian_curvature}
\end{align}
\normalsize
From \eqref{eq:riemannian_curvature}, we can see that curvature is determined by the connection $\Gamma^l_{ij}$.
Next, the Hessian of function on the manifold is defined as follows.
\begin{definition}
    \label{def:hessian}
    The Hessian $H^f$ of $f \in \mathcal{F}(\mathcal{M})$ with respect to the linear connection $\nabla$ is the covariant derivative of the $1$-form $df$ as
    %\begin{align}
        $H^f(X, Y) \coloneqq (\nabla df)(X, Y)$.
    %\end{align}
\end{definition}
We also have the explicit formula as $H^f(X, Y) = X df(Y) - df(\nabla_X Y) = XY(f) - (\nabla_X Y)f$,
and the local coordinates representation is
% \vspace{-2mm}
\small
\begin{align}
    H^f_{ij} = \frac{\partial^2 f}{\partial \theta^i \partial \theta^j} - \Gamma^k_{ij}\frac{\partial f}{\partial \theta^k}. \label{eq:hessian_local_coordinates}
\end{align}
% \normalsize
From \eqref{eq:riemannian_curvature} and \eqref{eq:hessian_local_coordinates}, it is obvious that studying on the Hessian is equivalent to the investigation of the Riemannian curvature tensor.
We also consider the following dual form, from the idea of information geometry
% ~\citep{amari2000methods,amari2016information,nielsen2020elementary}.
~\citep{amari2016information,nielsen2020elementary}.

\begin{definition}
    Let $\nabla, \nabla^*$ be a pair of torsion-free dual connections on the Riemannian manifold $(\mathcal{M}, \mathfrak{g})$.
    For each smooth function $f$ on $\mathcal{M}$, the dual Hessian $H^{*f}$ is given by $H^{*f} \coloneqq (\nabla^* df)(X, Y)$,
    and its components are $H^{*f}_{ij} = \frac{\partial^2 f}{\partial\theta_i\partial\theta_j} - \Gamma^{*k}_{ij}\frac{\partial f}{\partial\theta^k}$.
\end{definition}

Next, we give the following contractions of curvature.
\begin{definition}[Spectral radius]
    \label{def:spectral_radius}
    Let $\lambda_1,\dots,\lambda_m$ be the eigenvalues of Hessian $H^f$ for some function $f \in \mathcal{F}(\mathcal{M})$.
    The spectral radius of $H^f$ is defined as
    %\begin{align}
        $A(H^f) \coloneqq \max_{i \in [0, m]}\{|\lambda_1|,\dots,|\lambda_m|\}$,
    %\end{align}
    and $A(H^f) = \lim_{k\to\infty}\|H^{fk}\|^{1/k}$.
\end{definition}
\begin{definition}[Laplacian]
    For every linear connection $\nabla$, any metric $\mathfrak{g}$ and $C^2$-function $f$, Laplacian operator $\Delta f$ is defined as
    %\begin{align}
        $\Delta f = div(grad\ f)$,
    %\end{align}
    where $div$ is the divergence of vector field and $grad$ is the gradient vector field of $f$.
\end{definition}




\begin{figure*}[t]
\vspace{-3mm}
    \centering	
    \includegraphics[width=0.25\linewidth]{figs/fig3/CIFAR/avg_test_acc-vs-avg_test_ece}
    \includegraphics[width=0.26\linewidth]{figs/fig3/CIFAR/test_eigen_h-vs-avg_test_acc.pdf}
    \includegraphics[width=0.25\linewidth]{figs/fig3/CIFAR/test_eigen_h-vs-avg_test_ece.pdf}
\vspace{-3mm}
\caption{Effects of batch size variations on the behavior of SAM in the CIFAR10.1 task. Each color represents an experiment with a different batch size. With an appropriate batch size (BS=256), both ACC and ECE performance is good. BS=Full performs well only in terms of ECE, while BS=1 results in suboptimal performance for both indicators.}
\vspace{-6mm}
\label{fig:fig3}
\end{figure*}




Our interest lies in identifying the specific contractions among the aforementioned approximations that account for the common causal effect of curvature in algorithms known to be effective for existing OOD generalization and calibration.
To provide this, we consider the following lemmas.
\begin{lemma}
    \label{lemma:full_batch_sam}
    Full-batch SAM penalizes the scaled largest eigenvalues of Hessian at the rate of $\mathcal{O}(\eta\rho^2\ln(1 / \rho))$, for learning rate $\eta$ and perturbation radius $\rho$.
\end{lemma}
\begin{lemma}
    \label{lemma:1_batch_sam}
    1-batch SAM penalizes the trace of Hessian at the rate of $\mathcal{O}((\eta^{1/4 + \rho^{1/4}})\rho^2)$, for learning rate $\eta$ and perturbation radius $\rho$.
\end{lemma}
These are the results obtained for SAM~\citep{wen2023how}, and we also consider the relation between the Focal Loss and curvature as follows.
\vspace{-3mm}
\begin{proposition}
\label{prop:focal_loss_and_cross_entropy}
Let $p(y|\bm{x};\bm{\theta})$ be a model parameterized by $\bm{\theta}\in\Theta$ and $q(y|\bm{x})$ be a true distribution.
For $\gamma\geq 0$, we have
\small
\begin{align}
    \mathcal{L}^\gamma_f(\bm{\theta}) \geq \mathcal{L}_c(\bm{\theta}) - \gamma \mathcal{H}(y|\bm{x}, \bm{\theta}), \label{eq:focal_loss_and_cross_entropy}
\end{align}
\normalsize
where $\mathcal{L}_c(\bm{\theta}) = -\int_{\mathcal{X}\times\mathcal{Y}}q(y|\bm{x})\ln p(y|\bm{x};\bm{\theta})d\bm{x}dy$ is the cross-entropy loss and $\mathcal{H}(y|\bm{x},\bm{\theta})$ is the conditional entropy.
\end{proposition}
From \eqref{eq:focal_loss_and_cross_entropy}, learning procedure with Focal Loss can be regarded as maximizing conditional entropy term under the constraint
\footnotesize
\begin{align}
    \int_{\Theta} p(\bm{\theta})\mathcal{L}_c(\bm{\theta})d\theta &= \int_\Theta p(\bm{\theta})\left(-\int_{\mathcal{X}\times\mathcal{Y}}q(y|\bm{x})\ln p(y|\bm{x};\bm{\theta})d\bm{x}dy\right)d\bm{\theta} \nonumber\\
    &= \delta_\gamma \leq \delta, \label{eq:focal_loss_constraint}
\end{align}
\normalsize
for some $\delta\geq 0$ and $\delta_\gamma\geq 0$.
\begin{theorem}
\label{thm:maxwell_boltzmann}
Among all distributions defined on $\Theta$ with a given $\delta_\gamma$, the distribution with the largest entropy is the Maxwell-Boltzmann distribution
\small
\begin{align}
    \tilde{p}(\bm{\theta}) %&= \alpha\cdot e^{-\beta\cdot\mathcal{L}_c(\bm{\theta})} \nonumber\\
    &= \alpha\cdot\exp\left\{\beta\int_{\mathcal{X}\times\mathcal{Y}}q(y|\bm{x})\ln p(y|\bm{x};\bm{\theta})d\bm{x}dy\right\}, \label{eq:maxwell_boltzmann}
\end{align}
\normalsize
where the constants $\alpha$ and $\beta$ are determined from the following constraints
\footnotesize
\begin{align}
    \int_\Theta p(\bm{\theta})d\bm{\theta} = 1 &\Longleftrightarrow \alpha = \left(\int_\Theta e^{-\beta\cdot\mathcal{L}_c(\bm{\theta})}d\bm{\theta}\right)^{-1}, \label{eq:maxwell_boltzmann_const_1} \\
    \int_\Theta\mathcal{L}_c(\bm{\theta})p(\bm{\theta})d\bm{\theta} = \delta_\gamma &\Longleftrightarrow \int_\Theta \mathcal{L}_c(\bm{\theta})e^{-\beta\cdot\mathcal{L}_c(\bm{\theta})}d\bm{\theta} = \frac{\delta_\gamma}{\alpha} \label{eq:maxwell_boltzmann_const_2}.
\end{align}
\normalsize
\end{theorem}
Using \eqref{eq:maxwell_boltzmann} as the prior of parameter distribution as $\pi = \tilde{p}$, we give the following PAC-Bayes bound by using Thiemann's bound\citep{thiemann2017strongly}.
\begin{proposition}
\label{prop:pac_bayes_maxwell_boltzmann}
Maxwell-Boltzmann distribution induces the following bound
\footnotesize
\begin{align}
    \mathbb{P}\left[\forall{\varsigma}\in P(\Theta), \mathbb{E}_{\bm{\theta}\sim\varsigma}\left[\mathcal{R}(\bm{\theta})\right] \leq J(\zeta, \lambda) + \frac{D_{KL}[\varsigma\|\pi] + \ln\frac{2\sqrt{n}}{\epsilon}}{n\lambda(1-\frac{\lambda}{2})}\right] \leq \epsilon \nonumber\label{eq:pac_bayes_bound}
\end{align}
\normalsize
for some $\epsilon>0$ and $\lambda\geq 0$, where $J(\zeta, \lambda) = \frac{\mathbb{E}_{\bm{\theta}\sim\varsigma}[\hat{R}(\bm{\theta})]}{1 - \frac{\lambda}{2}}$.
The minimum of the right-hand side is achieved by
\footnotesize
\begin{align}
    \varsigma_\lambda(\bm{\theta}) &= \frac{\pi(\bm{\theta})e^{-\lambda n \hat{R}(\bm{\theta})}}{\mathbb{E}_{\bm{\theta}\sim\pi}\left[e^{-\lambda n \hat{R}(\bm{\theta})}\right]},\quad (\text{fixed $\lambda$}),\\
    \lambda &= \frac{2}{\sqrt{\frac{2n \mathbb{E}_\varsigma\left[\hat{\mathcal{R}}(\bm{\theta})\right]}{D_{KL}\left[\varsigma\|\pi\right] + \ln\frac{2\sqrt{n}}{\delta}} + 1} + 1}\quad (\text{fixed $\varsigma$}).
\end{align}
\normalsize
\end{proposition}
\begin{proposition}
    Focal Loss equips the following regularizer:
    \footnotesize
    \begin{align}
        D_{KL}[\varsigma\|\pi] &= \int_\Theta \varsigma(\bm{\theta})\ln\frac{\varsigma(\bm{\theta})}{c\cdot\exp\left\{\beta\int_{\mathcal{X}\times\mathcal{Y}}q(\bm{x},y)\ln p(y|\bm{x};\bm{\theta})\right\}}d\bm{\theta}. \nonumber
    \end{align}
    \normalsize
\end{proposition}
\begin{proposition}
    \label{prop:sharpness_focal_loss}
    Learning with Focal Loss reduces the local sharpness of the likelihood, if prior $\pi$ and posterior $\varsigma$ are close enough.
\end{proposition}
Since cross-entropy is the expectation of the negative log-likelihood function, we have the following remarks.
\begin{proposition}
    \label{prop:focal_loss_curvature}
    Focal Loss reduces the local curvature of the loss landscape.
\end{proposition}
See Appendix~\ref{apd:focal_loss_curvature} for the proofs of the above propositions.
From the above discussion, we obtain the following main theorem.
\begin{theorem}[Curvature contractions]
\label{thm:curvature_contractions}
    For some loss function $f \in \mathcal{F}(\mathcal{M})$, we have the following.
    \begin{itemize}
        \item[i)] Full-batch SAM behaves as the regularizer of spectral radius of $H^f$.
        \item[ii)] 1-batch SAM and Focal Loss behave as the regularizers of the Laplacian of $f$.
    \end{itemize}
\end{theorem}

\begin{proof}
First, from Lemma~\ref{lemma:full_batch_sam} and Definition~\ref{def:spectral_radius}, i) is obvious.
Next, from the definition of Hessian, gradient and dual connections, we have
\vspace{-2mm}
\small
\begin{align*}
    H^f(X, Y) &= X(Y(f)) - (\nabla_XY)f \\
    &= X\mathfrak{g}(grad\ f, Y) - \mathfrak{g}(grad\ f, \nabla_XY) \\
    &= \mathfrak{g}(\nabla^*_X(grad\ f), Y), \quad \forall X, Y \in \mathcal{X}(\mathcal{M}).
\end{align*}
\vspace{-2mm}
\normalsize
Similarly, we have
\small
\begin{align*}
    H^{*f}(X, Y) = \mathfrak{g}(\nabla_X(grad\ f), Y), \quad \forall X, Y \in \mathcal{X}(\mathcal{M}).
\end{align*}
\vspace{-2mm}
\normalsize
Taking the trace yields
\small
\begin{align*}
    \mathrm{tr}(H^{*f}) &= \mathrm{tr}((X, Y) \to \mathfrak{g}(\nabla_X(grad\ f), Y)) \\
    &= div(grad\ f) = \Delta f.
\end{align*}
\normalsize
Then, from Lemma~\ref{lemma:1_batch_sam} and Remark~\ref{prop:focal_loss_curvature}, we have ii).
\end{proof}
In addition, from the fact that $\mathrm{tr}(H^f) = \sum_i \lambda_i$ for eigenvalues $\lambda_i$ of $H^f$, we have the following corollaries.
\begin{corollary}
    \label{cor:one_batch_full_batch_sam}
    If loss landscape is locally convex around some point $p$, that is, $H^f$ is positive semidefinite, then the regularization term of full-batch SAM is upper bounded by the regularization term of 1-batch SAM with some scaling factor $c \in \mathbb{R}$, as $A(H^f) \leq c\Delta f$.
\end{corollary}
\begin{corollary}
    \label{cor:robustness_sam_focal}
    If the loss landscape has locally concave directions at some point $p$, full-batch SAM is more robust than 1-batch SAM or Focal Loss regularization.
\end{corollary}

Note that all the above theorems are asymptotic results.
Indeed, the discussion on SAM is for the learning rate and perturbation radius, and for Focal Loss, the focus is on the small variations of parameters.
While there may be potential discrepancies between these results and empirical observations, they provide suggestive insights in terms of unifying methods from a geometric perspective.
Appendix~\ref{apd:geometry},\ref{apd:focal_loss_curvature} and \ref{apd:additional_discussions} provide more details of theoretical investigation and additional discussions.

==> setup.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}

% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}
\usepackage{booktabs}
\usepackage{array}

\usepackage{url}
\usepackage{bm}
\usepackage{graphicx}
\usepackage{color}
\usepackage{here}

\usepackage[whole]{bxcjkjatype} % Japanese

\newcommand*{\TODO}[1]{{\colorbox{red}{\color{white}{#1}}}}
\newcommand*{\UPDATE}[1]{\textcolor{red}{#1}}
\newcommand*{\FIX}[1]{{\textcolor{green}{#1}}}
\newcommand*{\PREV}[1]{{\textcolor{gray}{#1}}}


\usepackage{amsthm}
\usepackage{mathtools}

\usepackage{lipsum}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{hypothesis}{Hypothesis}

\usepackage{cite}
\usepackage{ascmac}

\usepackage{markdown}
\usepackage{lipsum}

% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}


% Support for easy cross-referencing
\usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\Crefname{table}{Table}{Tables}
\crefname{table}{Tab.}{Tabs.}






%%%%%%%%% MATH COMMAND %%%%%%%%%


\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem{example}{Example}

